Deep PatchMatch MVS with Learned Patch Coplanarity, Geometric Consistency and Adaptive Pixel Sampling

Recent work in multi-view stereo (MVS) combines learnable photometric scores and regularization with PatchMatch-based optimization to achieve robust pixelwise estimates of depth, normals, and visibility. However, non-learning based methods still outperform for large scenes with sparse views, in part due to use of geometric consistency constraints and ability to optimize over many views at high resolution. In this paper, we build on learning-based approaches to improve photometric scores by learning patch coplanarity and encourage geometric consistency by learning a scaled photometric cost that can be combined with reprojection error. We also propose an adaptive pixel sampling strategy for candidate propagation that reduces memory to enable training on larger resolution with more views and a larger encoder. These modifications lead to 6-15% gains in accuracy and completeness on the challenging ETH3D benchmark, resulting in higher F1 performance than the widely used state-of-the-art non-learning approaches ACMM and ACMP.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> tex/abstract.tex <==
\abstract{
    
    Recent work in multi-view stereo (MVS) combines learnable photometric scores and regularization with PatchMatch-based optimization to achieve robust pixelwise estimates of depth, normals, and visibility.  However, non-learning based methods still outperform for large scenes with sparse views, in part due to use of geometric consistency constraints and ability to optimize over many views at high resolution.  In this paper, we build on learning-based approaches to improve photometric scores by learning patch coplanarity and encourage geometric consistency by learning a scaled photometric cost that can be combined with reprojection error. 
    We also propose an adaptive pixel sampling strategy for candidate propagation that reduces memory to enable training on larger resolution with more views and a larger encoder. These modifications lead to 6-15\% gains in accuracy and  completeness on the challenging ETH3D benchmark, resulting in higher $F_1$ performance than the widely used state-of-the-art non-learning approaches ACMM and ACMP.
    %Learning-based PatchMatch multiview stereo~(MVS) methods achieve have shown good performance, %combine 
    %with the advantage of %CNN-based feature extraction and 
    %an efficient CNN architecture for pixel-wise estimation. 
    %However, these methods are still %fail for scenes with texture-less regions and sparse views, %where non-learning based methods perform well due to their high-resolution input and guided priors such as coplanarity and geometric consistency. 
    %inferior to non-learning based approaches, partly due to indistinguishable local patch features, non-spatially aligned depth search in cost regularization, and limited input image resolution and number of views due to memory constraints.
    %To address these issues, in this paper, %to close the performance gap for learning-based PatchMatch MVS, 
    %we propose to model the pixel support for photometric scores by learning local patch coplanarity, and introduce geometry consistency to learning-based MVS for the first time, by rescaling the learned photometric scores to a log-disbelief estimation. We derive an adaptive pixel sampling strategy for candidate propagation, which allows high-res image input, more views and a denser backbone. Our method achieves state-of-the-art performance among learning-based MVS methods. Compared to the non-learning based architecture~(\eg~ACMM), we achieve a higher $F_1$ score on the challenging ETH3D high-res benchmark, and perform on-par on advanced TnT.
    %We provide extensive analysis on which modules are responsible for the improvement.
}
\keywords{Multi-View Stereo, Learning-based Stereo, 3D Reconstruction}



==> tex/method_backup.tex <==
\input{figures/architecture}
\section{Method}
%In this section, we describe our approach in detail. 
Figure~\ref{fig:architecture} shows an overview of our architecture during training. We build our approach on PatchMatch-RL~(Sec.~\ref{method:PMRL}), a recent learning-based PatchMatch MVS framework, and propose three designs that lead to large performance gain in both accuracy and completeness: (1) improve the photometric cost function by directly modeling the coplanarity of neighboring pixels~(Sec.~\ref{method:coplanarity}); (2) replace the recurrent cost regularization with geometric consistency by learning a scaled photometric cost ~(Sec.~\ref{method:gc}); (3) design an adaptive pixel sampling strategy for candidate propagation to reduce memory, so that high-res images, more views, and deeper features can be used for training~(Sec.~\ref{method:adaptive}).

%Our method adopts the training and the inference architecture of PatchMatch-RL, with four additional modifications. First, we replace the dot-product attention with the jointly trained pixel-wise coplanar weights. Next, we use UNet~\cite{ronneberger2015u}-shaped feature extractor trained with subset of adaptively selected supporting pixels for memory efficiency. Then, we add geometric-consistency based regularization in inference time, allowing more complete reconstruction. 

\subsection{Review of PatchMatch-RL}\label{method:PMRL}
The input of PatchMatch-RL is a set of reference and source images $\{I_r, I_i\}^N_{i=1} \subset \mathcal{I}$, and their corresponding cameras poses $\{C_r, C_i = (K_i, R_i, t_i)\}^N_{i=1} \subset \mathcal{C}$ including intrinsic and extrinsic parameters. %where $\mathcal{I}, \mathcal{C}$ represents all set of images and cameras in the scene, $I_1, C_1$ represents reference image and camera, and $(K_i, R_i, t_i) = C_i$ represents intrinsic, extrinsic rotation and extrinsic translation of the $i$-th camera, 
The method uses a coarse-to-fine PatchMatch MVS inference to jointly estimate the depths, normals, and visiblities of the reference image $D_r, N_r, \{V_{r,i}\}^N_{i=1}$, and uses policy-gradient for end-to-end training.

PatchMatch-RL starts by extracting CNN based features $\{f^{\theta}(I_r), f^{\theta}(I_i) = F^{s}_i\}^N_{i=1}$ at multiple scales $s \in \{3, 2, 1\}$, where $f^{\theta}$ represents trainable CNN backbone with parameters $\theta$, and $s$ represents the $\log_2$ scale resolution of the image (\eg $F^s_i \rightarrow \mathbb{R}^{\frac{H}{2^s} \times \frac{W}{2^s} \times C}$). Then, the method initializes the depth and normal map $d^{s,t}_r,n^{s,t}_r$ at the coarsest scale $s=3$ and the initial iteration $t=0$.
For the ease of notation, we drop the scale $s$ and let $d^t_r, n^t_r, v^t_{r,i}$ denote the depth, normal and visibility map at the $t$-th iteration on the same scale in the coarse-to-fine stage from onward. 

After initialization, a series of PatchMatch iterations are run at each scale, and each iteration jointly updates the depth, normal, and visibility maps. A single PatchMatch iteration consists of 4 steps: 
\begin{enumerate}
    \item \textbf{Pixel-wise view selection} updates the visiblity map $v^{t}_{r, i} \rightarrow v^{t+1}_{r, i}$ using the current set of depth $d^{t}_r$ and normal $n^{t}_r$ scored by an MLP, which defines the parameterized view-sampling policy $\pi^v_\theta$.
    \item \textbf{Candidate Propagation} generates potential candidates of depth and normal for the next iteration by using PatchMatch-based propagation. 
    \item \textbf{Candidate Scoring} scores each candidate depth / normal pairs using the current set of visibility map $v^{t+1}_{r, i}$ through an RNN-based scorer regularizer which defines the parameterized candidate-sampling policy $\pi^s_\theta$.
    \item \textbf{Candidate Selection} updates the current depth and normal map to $d^{t+1}_r$ and $n^{t+1}_r$,
\end{enumerate}
\input{figures/inference}

The parameterized policies represents the sampling procedure defined by the distribution formed by the scores obtained by the MLP and the RNN. 
In inference, the policy performs arg-max selection based on the set of computed scores. In training, the policy performs selection based on the decaying $\epsilon$-greedy method, where it samples from the distribution with the probability of $\epsilon$ and samples using arg-max with the probability of $1-\epsilon$. 

After a sufficient number of iterations for each scale, the depth and normal maps are upscaled using nearest neighbor upsampling. Then, the next stage of the coarse-to-fine architecture starts, and the process is repeated until the most finest-level iteration is completed.

To train the model in an end-to-end differentiable manner, PatchMatch-RL uses policy-gradient algorithm REINFORCE to jointly train $f^\theta, \pi^v_\theta, \pi^s_\theta$. %This is because the PatchMatch iteration contains hard-selection of candidate (either through the arg-max, or through the sampling) depth and normal pairs, which is not differentiable.
The reward for each iteration is defined as $r^t = \mathcal{N}(d^t_r; D^*_r, \sigma_d) \cdot \mathcal{N}(n^t_r; N^*_r, \sigma_n)$, where $D^*_r$ and $N^*_r$ represent the ground-truth depth and normal maps, and $\mathcal{N}(x; \mu, \sigma)$ represents the probability of observing $x$ from the normal distribution with mean $\mu$ and standard deviation $\sigma$. 
%PatchMatch-RL trains the model using the REINFORCE 
The update for each iteration is:
\begin{align}
    \triangledown_\theta J &=  \sum_t \sum_{t'>=t} \triangledown_\theta \gamma^{t'-t} r^t \log \pi_\theta.
\end{align}
We let $\gamma$ represent the discount coefficient of future reward. PatchMatch-RL additionally modifies the candidate selection loss to use cross-entropy between the ground-truth distribution of observing each candidate (\eg $\forall (d, n), \mathcal{N}(d; D^*_r, \sigma_d) \cdot \mathcal{N}(n; N^*_r, \sigma_n)$) and the distribution formed by the scores of each candidates using the candidate scoring policy for robustness in training. 
\input{figures/coplanarity}
\input{figures/coplanarity_comparison}
\subsection{Learning Patch Coplanarity}\label{method:coplanarity}

Estimating the surface normal for each pixel requires a patch-based photometric score, computed as a weighted sum of similarities over supporting interpolated feature positions.  Rather than computing weights using scaled dot-product attention like PatchMatch-RL, we propose to set the weights to the likelihood of coplanarity with supporting pixels, which is estimated using a separate CNN architecture.
%Instead, we propose to directly estimate the coplanarity of each pixels by using a separate CNN architecture. 
%We modify the CSPN~\cite{cheng2019learning} architecture , which learns the affinity of neighboring points, to learn the corresponding similarity values for the supporting pixels. 
We modify the CSPN architecture~\cite{cheng2019learning} used to learn the affinity of neighboring points, and change its last layer to a $3\times 3$ convolution with a dilation of 3, so that the receptive field matches the supporting pixel weight locations.
Figure~\ref{fig:coplanar} depicts an overview of our coplanarity extraction and output feature representation. We train the coplanarity by policy gradient loss from the coplanar-weighted visibility and candidate scores, along with an additional mean square error loss term obtained from the ground-truth coplanarity points obtained from the ground-truth depth. We show in Figure~\ref{fig:coplanar-comparison} that compared with existing supporting pixel weighting schemes, our approach can better identify coplanarity within local patches with different textures.

\subsection{Encouraging Geometric Consistency in Inference}\label{method:gc}
% PatchMatch-RL uses recurrent cost regularization to regularize cost over the PatchMatch iterations. Although the recurrent cost regularization has shown improvement over the pure MLP-based scoring function, it does not fully utilize neighborhood scores like the cost-volume based regularization~\cite{yao2018mvsnet, yao2019recurrent}. 
% This is because the PatchMatch propagated geometry is not spatially aligned, and also partly because the propagated geometry contains normals which make it impossible to perform aligned grid search like the methods that perform depth only search. 
% Instead
We propose geometric consistency based regularization %used in the non-learning based PatchMatch MVS methods~\cite{schoenberger2016mvs, xu2019multi}, 
to replace the recurrent cost regularization used in PatchMatch-RL. The key idea of geometric consistency is to use the inferred geometry of the source images to validate the reference image geometry. We adopt the geometric consistency score used in ACMM~\cite{xu2019multi}, which defines an additional score term based on the reprojection error of the visible source view pixels.

Although geometric consistency is commonly used for non-learning based approaches~\cite{schoenberger2016mvs,xu2019multi}, it is challenging to integrate in learning-based approaches, since the source view geometry is not differentiable with respect to the reference view geometry. %In order to integrate geometric consistency scores into the learned photometric scores $S_{pho}(p)$, 
%In order to allow the optional addition of additional geometric logarithmic suspicion scores in the candidate selection stage, without having to train additional modules to combine the two scores, we remap the photometric score and geometric consistency score range to the logarithmic suspicion range.
In order to allow the optional adding of geometric log-disbelief scores in candidate selection stage without having to train additional module to combine the two scores, we remap the photometric score and the geometric consistency score range to the log-disbelief range. 
In detail, we let the photometric score ranges logarithmically from $0$ to $S_{max}$, where $0$ implies perfect photometric match and $S_{max}$ implies complete disagreement.
%Instead of using RNN, 
We use MLP as the photometric consistency scorer to replace the RNN-based scorer, since the history of candidate selection cannot handle the additional geometric consistency term in inference. 

We let the pixel-wise reprojection error distance be the log scale disbelief score of the geometric consistency term.
Given the candidate depth and normal map $d_\phi, n_\phi = \phi$, we use the homography between image $j$ and image $k$ at pixel $p$ defined as $H_{j \rightarrow k}(p) = K_k \cdot (R_{j\rightarrow k} - \frac{t_{j\rightarrow k} \cdot n^T_j(p)}{d_j(p)}) \cdot K^{-1}_j$, and compute the reprojection error:
\begin{equation}
    E_{\phi\rightarrow i}(p) = || H_{i \rightarrow \phi}(H_{\phi\rightarrow i}(p) \cdot p) -  p ||_2
\end{equation}
We define $G_{max}$ as the maximum log-disbelief term that can be added to geometric consistency, and combine the score weighted by the visibility mapping weights:
\begin{equation}
    S^{\phi}_{geo}(p) = \sum^{N}_{i=2} v^t_i \cdot (S^{\phi}_{pho}(p) + \min(E_{\phi\rightarrow i}(p), G_{max}))
\end{equation}
We then use $S^\phi_{geo}(p)$ to select candidate for the pixel $p$, updating the depth $d_r(p)$ and normal $n_r(p)$ at the corresponding iteration.

Since we need to have the source view geometry available to use geometric consistency based regularization, we use a modified version of the coarse-to-fine architecture, as illustrated in Figure~\ref{fig:inference}.
%In the coarse to fine reconstruction with geometric consistency, 
In inference, the source view and its inferred geometry in the previous stage are used to calculate $S^{\phi}_{geo}$ for the candidate selection step of each PatchMatch iteration. The inferred depth and normal maps at each stage are stored in a file, and loaded in the next stage of reconstruction with geometric consistency.


% \input{tables/tanks_and_temples}
\subsection{Adaptive Supporting Pixel Sampling}\label{method:adaptive}
Training the learning based PatchMatch MVS model using policy gradient requires memory linear to the number of depth, normal and visibility map evaluations (\eg number of PatchMatch iterations), since the history of gradients need to be stored. 
Hence, PatchMatch-RL~\cite{lee2021patchmatchrl} uses shallow VGG-style backbone, with a small number of PatchMatch iterations per scale. 
We resolve this problem by using a sampled subset of the supporting pixels in training, which effectively reduces the number of computation used during training time by half and the memory used by around 30\%, so that a larger feature extraction backbone can be used with faster training. 
We use the distribution of the coplanar value of the supporting pixels as a sampling distribution. 
We sample 3 points out of 8 supporting pixels, (excluding the center pixel of the $3\times 3$ local supporting pixels), which is the minimum number of points that ensures surface normal orientation. 
The adaptive supporting pixel sampling can be used in the inference time for faster runtime, at the cost of a slight drop in reconstruction quality. We attach a detailed analysis in the supplementary material. 
% Table~\ref{tab:ablation} in Section~\ref{sec:experiments} shows the detailed analysis of the effect of adaptive supporting pixel sampling in inference. 

==> tex/review.tex <==
\section{Review of PatchMatch-RL}
